Complexity of equilibria in binary public goods games on undirected graphs

We study the complexity of computing equilibria in binary public goods games on undirected graphs. In such a game, players correspond to vertices in a graph and face a binary choice of performing an action, or not. Each player's decision depends only on the number of neighbors in the graph who perform the action and is encoded by a per-player binary pattern. We show that games with decreasing patterns (where players only want to act up to a threshold number of adjacent players doing so) always have a pure Nash equilibrium and that one is reached from any starting profile by following a polynomially bounded sequence of best responses. For non-monotonic patterns of the form $10^k10^*$ (where players want to act alone or alongside $k + 1$ neighbors), we show that it is $\mathsf{NP}$-hard to decide whether a pure Nash equilibrium exists. We further investigate a generalization of the model that permits ties of varying strength: an edge with integral weight $w$ behaves as $w$ parallel edges. While, in this model, a pure Nash equilibrium still exists for decreasing patters, we show that the task of computing one is $\mathsf{PLS}$-complete.

==> tikz_header.tex <==
\tikzset{
    node distance=6mm,
    public/.style={circle, fill=black, scale=0.5},
    membrane/.style={circle, draw=black, fill=lightgray, scale=0.5},
    private/.style={circle, draw, scale=0.5},
    hidden/.style={circle, scale=0.5},
    leftout/.style={dotted, thick},
    box/.style={draw, rectangle, inner sep=0.75mm, rounded corners=1mm},
    group/.style={box, draw=lightgray},
}

